Many-Joint Robot Arm Control with Recurrent Spiking Neural Networks

In the paper, we show how scalable, low-cost trunk-like robotic arms can be constructed using only basic 3D-printing equipment and simple electronics. The design is based on uniform, stackable joint modules with three degrees of freedom each. Moreover, we present an approach for controlling these robots with recurrent spiking neural networks. At first, a spiking forward model learns motor-pose correlations from movement observations. After training, intentions can be projected back through unrolled spike trains of the forward model essentially routing the intention-driven motor gradients towards the respective joints, which unfolds goal-direction navigation. We demonstrate that spiking neural networks can thus effectively control trunk-like robotic arms with up to 75 articulated degrees of freedom with near millimeter accuracy.

==> figures/pseudoshape/spiketrain.tex <==
\addplot[mark=*, only marks,mark size=0.7pt,color=black] plot coordinates {
(1,93)
(1,108)
(1,379)
(1,461)
(1,475)
(2,46)
(2,63)
(2,71)
(2,73)
(2,78)
(2,89)
(2,132)
(2,145)
(2,162)
(2,197)
(2,210)
(2,223)
(2,227)
(2,232)
(2,235)
(2,246)
(2,250)
(2,253)
(2,273)
(2,285)
(2,286)
(2,298)
(2,305)
(2,326)
(2,361)
(2,370)
(2,399)
(2,409)
(2,415)
(2,471)
(3,1)
(3,2)
(3,5)
(3,7)
(3,8)
(3,10)
(3,15)
(3,16)
(3,22)
(3,25)
(3,26)
(3,34)
(3,35)
(3,38)
(3,39)
(3,51)
(3,53)
(3,56)
(3,65)
(3,68)
(3,69)
(3,70)
(3,81)
(3,88)
(3,106)
(3,107)
(3,115)
(3,116)
(3,119)
(3,120)
(3,126)
(3,136)
(3,155)
(3,156)
(3,158)
(3,159)
(3,161)
(3,173)
(3,174)
(3,175)
(3,177)
(3,183)
(3,195)
(3,200)
(3,202)
(3,213)
(3,221)
(3,237)
(3,238)
(3,239)
(3,244)
(3,274)
(3,276)
(3,288)
(3,289)
(3,290)
(3,308)
(3,313)
(3,316)
(3,320)
(3,331)
(3,341)
(3,344)
(3,354)
(3,368)
(3,371)
(3,374)
(3,381)
(3,387)
(3,395)
(3,402)
(3,403)
(3,410)
(3,412)
(3,417)
(3,428)
(3,429)
(3,432)
(3,452)
(3,458)
(3,459)
(3,464)
(3,465)
(3,476)
(3,485)
(3,488)
(3,491)
(3,499)
(3,500)
(3,502)
(3,505)
(4,3)
(4,42)
(4,50)
(4,58)
(4,103)
(4,117)
(4,123)
(4,139)
(4,149)
(4,179)
(4,184)
(4,189)
(4,194)
(4,259)
(4,300)
(4,311)
(4,338)
(4,348)
(4,356)
(4,365)
(4,390)
(4,392)
(4,398)
(4,404)
(4,420)
(4,431)
(4,441)
(4,445)
(4,496)
(5,47)
(5,72)
(5,455)
(5,463)
(6,163)
(6,229)
(6,249)
(6,278)
(6,303)
(6,321)
(6,396)
(6,483)
(7,32)
(7,318)
(7,469)
(7,480)
(8,71)
(8,89)
(8,104)
(8,132)
(8,150)
(8,162)
(8,197)
(8,210)
(8,223)
(8,235)
(8,246)
(8,273)
(8,298)
(8,355)
(8,471)
(9,1)
(9,5)
(9,7)
(9,10)
(9,15)
(9,16)
(9,22)
(9,25)
(9,26)
(9,34)
(9,35)
(9,38)
(9,51)
(9,53)
(9,65)
(9,68)
(9,69)
(9,70)
(9,81)
(9,88)
(9,106)
(9,107)
(9,112)
(9,115)
(9,119)
(9,120)
(9,126)
(9,136)
(9,155)
(9,156)
(9,158)
(9,159)
(9,161)
(9,173)
(9,174)
(9,175)
(9,183)
(9,195)
(9,200)
(9,202)
(9,221)
(9,237)
(9,238)
(9,239)
(9,242)
(9,244)
(9,274)
(9,276)
(9,288)
(9,289)
(9,290)
(9,308)
(9,313)
(9,320)
(9,331)
(9,341)
(9,354)
(9,368)
(9,381)
(9,387)
(9,395)
(9,402)
(9,403)
(9,410)
(9,412)
(9,417)
(9,428)
(9,429)
(9,432)
(9,458)
(9,459)
(9,464)
(9,465)
(9,488)
(9,499)
(9,500)
(9,502)
(10,3)
(10,8)
(10,43)
(10,58)
(10,117)
(10,122)
(10,123)
(10,130)
(10,139)
(10,149)
(10,166)
(10,177)
(10,179)
(10,184)
(10,189)
(10,194)
(10,203)
(10,205)
(10,227)
(10,241)
(10,259)
(10,324)
(10,333)
(10,336)
(10,338)
(10,339)
(10,343)
(10,365)
(10,373)
(10,376)
(10,383)
(10,390)
(10,392)
(10,398)
(10,404)
(10,441)
(10,445)
(10,490)
(11,9)
(11,21)
(11,42)
(11,47)
(11,50)
(11,72)
(11,79)
(11,144)
(11,199)
(11,232)
(11,297)
(11,310)
(11,314)
(11,340)
(11,350)
(11,356)
(11,431)
(11,454)
(11,455)
(11,463)
(12,73)
(12,163)
(12,178)
(12,186)
(12,229)
(12,249)
(12,321)
(12,396)
(12,483)
(13,11)
(13,32)
(13,55)
(13,170)
(13,213)
(13,263)
(13,318)
(13,319)
(13,422)
(13,480)
(14,48)
(14,67)
(14,89)
(14,104)
(14,150)
(14,162)
(14,210)
(14,223)
(14,235)
(14,246)
(14,266)
(14,273)
(14,293)
(14,298)
(14,300)
(14,349)
(14,355)
(14,471)
(15,1)
(15,5)
(15,7)
(15,10)
(15,15)
(15,22)
(15,25)
(15,34)
(15,35)
(15,38)
(15,51)
(15,53)
(15,60)
(15,65)
(15,68)
(15,69)
(15,70)
(15,88)
(15,106)
(15,107)
(15,112)
(15,115)
(15,119)
(15,120)
(15,126)
(15,136)
(15,155)
(15,156)
(15,159)
(15,161)
(15,173)
(15,174)
(15,175)
(15,183)
(15,195)
(15,200)
(15,202)
(15,215)
(15,221)
(15,237)
(15,238)
(15,239)
(15,242)
(15,244)
(15,250)
(15,274)
(15,276)
(15,288)
(15,289)
(15,290)
(15,292)
(15,313)
(15,328)
(15,331)
(15,341)
(15,354)
(15,368)
(15,381)
(15,387)
(15,395)
(15,402)
(15,403)
(15,410)
(15,412)
(15,429)
(15,432)
(15,458)
(15,459)
(15,464)
(15,465)
(15,488)
(15,499)
(15,500)
(16,3)
(16,24)
(16,58)
(16,117)
(16,130)
(16,139)
(16,149)
(16,166)
(16,177)
(16,179)
(16,182)
(16,184)
(16,189)
(16,194)
(16,227)
(16,291)
(16,324)
(16,336)
(16,338)
(16,339)
(16,343)
(16,353)
(16,365)
(16,373)
(16,383)
(16,390)
(16,392)
(16,398)
(16,404)
(16,417)
(16,441)
(16,445)
(16,490)
(17,9)
(17,21)
(17,42)
(17,72)
(17,76)
(17,79)
(17,95)
(17,199)
(17,232)
(17,297)
(17,310)
(17,314)
(17,340)
(17,350)
(17,370)
(17,431)
(17,454)
(18,116)
(18,140)
(18,178)
(18,186)
(18,229)
(18,302)
(18,321)
(18,483)
(19,11)
(19,32)
(19,50)
(19,55)
(19,64)
(19,85)
(19,151)
(19,163)
(19,213)
(19,318)
(19,391)
(19,422)
(19,480)
(19,493)
(20,104)
(20,150)
(20,162)
(20,210)
(20,223)
(20,246)
(20,266)
(20,273)
(20,298)
(20,300)
(20,463)
(20,471)
(20,511)
(21,1)
(21,5)
(21,7)
(21,10)
(21,15)
(21,22)
(21,25)
(21,34)
(21,35)
(21,38)
(21,51)
(21,65)
(21,68)
(21,69)
(21,70)
(21,88)
(21,98)
(21,106)
(21,107)
(21,115)
(21,126)
(21,136)
(21,144)
(21,155)
(21,156)
(21,161)
(21,173)
(21,174)
(21,175)
(21,183)
(21,200)
(21,202)
(21,221)
(21,237)
(21,238)
(21,239)
(21,242)
(21,244)
(21,265)
(21,274)
(21,276)
(21,288)
(21,289)
(21,313)
(21,328)
(21,341)
(21,354)
(21,368)
(21,376)
(21,381)
(21,387)
(21,395)
(21,402)
(21,403)
(21,410)
(21,412)
(21,429)
(21,432)
(21,455)
(21,458)
(21,464)
(21,465)
(21,488)
(21,500)
(22,3)
(22,58)
(22,73)
(22,117)
(22,177)
(22,179)
(22,182)
(22,184)
(22,189)
(22,194)
(22,205)
(22,227)
(22,231)
(22,236)
(22,291)
(22,324)
(22,338)
(22,339)
(22,343)
(22,353)
(22,365)
(22,373)
(22,383)
(22,384)
(22,390)
(22,392)
(22,398)
(22,441)
(22,445)
(23,21)
(23,31)
(23,42)
(23,79)
(23,95)
(23,112)
(23,119)
(23,190)
(23,199)
(23,222)
(23,232)
(23,310)
(23,356)
(23,370)
(23,431)
(24,6)
(24,8)
(24,16)
(24,27)
(24,37)
(24,43)
(24,140)
(24,229)
(24,255)
(24,278)
(24,374)
(24,394)
(24,409)
(24,485)
(24,496)
(25,11)
(25,40)
(25,47)
(25,50)
(25,54)
(25,55)
(25,56)
(25,64)
(25,66)
(25,75)
(25,85)
(25,116)
(25,149)
(25,151)
(25,160)
(25,166)
(25,185)
(25,197)
(25,213)
(25,269)
(25,290)
(25,302)
(25,318)
(25,320)
(25,336)
(25,355)
(25,391)
(25,404)
(25,422)
(25,423)
(25,468)
(25,493)
(26,104)
(26,139)
(26,150)
(26,162)
(26,163)
(26,210)
(26,223)
(26,246)
(26,270)
(26,273)
(26,298)
(26,300)
(26,396)
(26,511)
(27,1)
(27,5)
(27,7)
(27,10)
(27,15)
(27,22)
(27,25)
(27,34)
(27,35)
(27,38)
(27,51)
(27,65)
(27,69)
(27,88)
(27,98)
(27,106)
(27,107)
(27,115)
(27,126)
(27,136)
(27,155)
(27,156)
(27,161)
(27,173)
(27,174)
(27,175)
(27,183)
(27,200)
(27,202)
(27,221)
(27,237)
(27,238)
(27,239)
(27,244)
(27,265)
(27,274)
(27,276)
(27,288)
(27,289)
(27,313)
(27,341)
(27,354)
(27,381)
(27,402)
(27,403)
(27,410)
(27,412)
(27,429)
(27,432)
(27,455)
(27,458)
(27,464)
(27,465)
(27,479)
(27,488)
(27,500)
(28,3)
(28,58)
(28,117)
(28,154)
(28,177)
(28,179)
(28,184)
(28,189)
(28,194)
(28,227)
(28,231)
(28,236)
(28,282)
(28,291)
(28,293)
(28,324)
(28,338)
(28,339)
(28,343)
(28,353)
(28,365)
(28,373)
(28,383)
(28,387)
(28,390)
(28,392)
(28,398)
(28,445)
(28,456)
(29,21)
(29,31)
(29,42)
(29,79)
(29,95)
(29,112)
(29,199)
(29,222)
(29,232)
(29,348)
(29,356)
(29,431)
(30,8)
(30,16)
(30,27)
(30,37)
(30,119)
(30,140)
(30,255)
(30,278)
(30,331)
(30,376)
(30,485)
(30,496)
(31,11)
(31,36)
(31,40)
(31,55)
(31,66)
(31,75)
(31,116)
(31,151)
(31,185)
(31,213)
(31,256)
(31,290)
(31,318)
(31,320)
(31,336)
(31,347)
(31,355)
(31,391)
(31,404)
(31,422)
(31,493)
(32,64)
(32,102)
(32,104)
(32,139)
(32,150)
(32,162)
(32,163)
(32,209)
(32,210)
(32,211)
(32,223)
(32,246)
(32,249)
(32,257)
(32,259)
(32,270)
(32,273)
(32,300)
(32,396)
(32,511)
(33,1)
(33,5)
(33,7)
(33,15)
(33,22)
(33,25)
(33,34)
(33,35)
(33,38)
(33,51)
(33,65)
(33,69)
(33,88)
(33,98)
(33,106)
(33,107)
(33,115)
(33,122)
(33,126)
(33,136)
(33,156)
(33,161)
(33,174)
(33,175)
(33,183)
(33,200)
(33,202)
(33,203)
(33,221)
(33,237)
(33,238)
(33,239)
(33,244)
(33,274)
(33,276)
(33,288)
(33,302)
(33,354)
(33,381)
(33,402)
(33,403)
(33,410)
(33,412)
(33,429)
(33,432)
(33,455)
(33,465)
(33,479)
(33,488)
(33,499)
(33,500)
(34,3)
(34,46)
(34,58)
(34,117)
(34,177)
(34,179)
(34,184)
(34,189)
(34,194)
(34,206)
(34,229)
(34,282)
(34,291)
(34,324)
(34,338)
(34,339)
(34,343)
(34,350)
(34,353)
(34,365)
(34,373)
(34,383)
(34,387)
(34,390)
(34,392)
(34,398)
(34,445)
(35,21)
(35,42)
(35,72)
(35,79)
(35,112)
(35,138)
(35,199)
(35,222)
(35,232)
(35,297)
(35,348)
(35,356)
(35,395)
(35,431)
(36,37)
(36,45)
(36,76)
(36,166)
(36,277)
(36,329)
(36,331)
(36,376)
(36,480)
(37,36)
(37,43)
(37,55)
(37,66)
(37,75)
(37,95)
(37,116)
(37,151)
(37,158)
(37,178)
(37,185)
(37,290)
(37,318)
(37,336)
(37,347)
(37,349)
(37,355)
(37,391)
(37,404)
(37,422)
(37,451)
(37,464)
(37,474)
(37,490)
(37,493)
(38,0)
(38,9)
(38,11)
(38,24)
(38,49)
(38,64)
(38,67)
(38,102)
(38,104)
(38,150)
(38,201)
(38,205)
(38,209)
(38,210)
(38,215)
(38,223)
(38,236)
(38,243)
(38,246)
(38,257)
(38,259)
(38,263)
(38,270)
(38,273)
(38,300)
(38,328)
(38,396)
(38,510)
(38,511)
(39,1)
(39,5)
(39,7)
(39,15)
(39,22)
(39,25)
(39,32)
(39,34)
(39,35)
(39,38)
(39,51)
(39,65)
(39,69)
(39,88)
(39,98)
(39,106)
(39,107)
(39,115)
(39,122)
(39,126)
(39,133)
(39,140)
(39,154)
(39,156)
(39,161)
(39,170)
(39,174)
(39,175)
(39,182)
(39,183)
(39,200)
(39,202)
(39,203)
(39,221)
(39,235)
(39,237)
(39,238)
(39,239)
(39,244)
(39,265)
(39,276)
(39,288)
(39,302)
(39,354)
(39,381)
(39,403)
(39,410)
(39,412)
(39,429)
(39,432)
(39,454)
(39,488)
(39,499)
(39,500)
(40,3)
(40,46)
(40,117)
(40,162)
(40,163)
(40,177)
(40,179)
(40,184)
(40,189)
(40,194)
(40,229)
(40,282)
(40,291)
(40,324)
(40,338)
(40,339)
(40,343)
(40,350)
(40,353)
(40,358)
(40,365)
(40,373)
(40,383)
(40,390)
(40,392)
(40,398)
(40,445)
(41,21)
(41,42)
(41,79)
(41,112)
(41,199)
(41,222)
(41,232)
(41,297)
(41,356)
(41,395)
(41,431)
(42,37)
(42,136)
(42,166)
(42,341)
(42,387)
(42,480)
(43,36)
(43,43)
(43,55)
(43,66)
(43,75)
(43,116)
(43,151)
(43,178)
(43,185)
(43,318)
(43,336)
(43,347)
(43,376)
(43,384)
(43,391)
(43,422)
(43,464)
(43,492)
(43,501)
(44,0)
(44,11)
(44,49)
(44,64)
(44,76)
(44,83)
(44,103)
(44,104)
(44,150)
(44,190)
(44,205)
(44,209)
(44,210)
(44,223)
(44,231)
(44,243)
(44,246)
(44,257)
(44,263)
(44,268)
(44,270)
(44,300)
(44,328)
(44,349)
(44,441)
(44,490)
(44,511)
(45,1)
(45,7)
(45,15)
(45,22)
(45,25)
(45,34)
(45,35)
(45,38)
(45,58)
(45,65)
(45,88)
(45,98)
(45,106)
(45,107)
(45,115)
(45,133)
(45,154)
(45,156)
(45,161)
(45,165)
(45,170)
(45,174)
(45,175)
(45,183)
(45,202)
(45,203)
(45,204)
(45,221)
(45,235)
(45,237)
(45,239)
(45,244)
(45,265)
(45,276)
(45,288)
(45,302)
(45,354)
(45,381)
(45,403)
(45,412)
(45,429)
(45,432)
(45,454)
(45,488)
(45,499)
(45,500)
(46,46)
(46,117)
(46,140)
(46,162)
(46,179)
(46,189)
(46,282)
(46,291)
(46,339)
(46,343)
(46,353)
(46,365)
(46,375)
(46,383)
(46,390)
(46,398)
(46,445)
(46,472)
(47,21)
(47,42)
(47,79)
(47,85)
(47,158)
(47,177)
(47,199)
(47,219)
(47,222)
(47,356)
(47,395)
(47,431)
(48,6)
(48,31)
(48,37)
(48,56)
(48,136)
(48,197)
(48,341)
(48,480)
(49,16)
(49,36)
(49,43)
(49,66)
(49,112)
(49,151)
(49,178)
(49,185)
(49,269)
(49,290)
(49,318)
(49,336)
(49,347)
(49,391)
(49,394)
(49,409)
(49,422)
(49,492)
(49,496)
(50,0)
(50,11)
(50,49)
(50,83)
(50,103)
(50,104)
(50,116)
(50,150)
(50,160)
(50,190)
(50,209)
(50,210)
(50,223)
(50,231)
(50,246)
(50,257)
(50,263)
(50,268)
(50,270)
(50,300)
(50,329)
(50,355)
(50,373)
(50,441)
(50,504)
(50,511)
(51,7)
(51,15)
(51,22)
(51,25)
(51,34)
(51,35)
(51,38)
(51,40)
(51,65)
(51,75)
(51,88)
(51,98)
(51,106)
(51,115)
(51,133)
(51,144)
(51,154)
(51,156)
(51,161)
(51,165)
(51,174)
(51,175)
(51,181)
(51,183)
(51,198)
(51,202)
(51,203)
(51,204)
(51,205)
(51,221)
(51,235)
(51,237)
(51,239)
(51,244)
(51,265)
(51,276)
(51,288)
(51,302)
(51,320)
(51,324)
(51,354)
(51,381)
(51,403)
(51,423)
(51,429)
(51,432)
(51,488)
(51,499)
(51,500)
(52,46)
(52,117)
(52,148)
(52,162)
(52,179)
(52,189)
(52,226)
(52,282)
(52,291)
(52,339)
(52,343)
(52,353)
(52,365)
(52,375)
(52,383)
(52,390)
(52,433)
(52,445)
(52,472)
(53,12)
(53,21)
(53,42)
(53,54)
(53,79)
(53,158)
(53,164)
(53,199)
(53,219)
(53,222)
(53,240)
(53,356)
(53,376)
(53,398)
(53,431)
(54,31)
(54,37)
(54,56)
(54,197)
(55,16)
(55,36)
(55,43)
(55,66)
(55,112)
(55,136)
(55,138)
(55,140)
(55,151)
(55,178)
(55,185)
(55,289)
(55,290)
(55,318)
(55,336)
(55,347)
(55,348)
(55,391)
(55,404)
(55,422)
(55,492)
(56,0)
(56,11)
(56,49)
(56,69)
(56,83)
(56,102)
(56,103)
(56,104)
(56,122)
(56,150)
(56,195)
(56,210)
(56,211)
(56,223)
(56,231)
(56,241)
(56,243)
(56,246)
(56,257)
(56,263)
(56,268)
(56,270)
(56,300)
(56,329)
(56,331)
(56,341)
(56,355)
(56,371)
(56,511)
(57,15)
(57,22)
(57,25)
(57,30)
(57,34)
(57,35)
(57,38)
(57,45)
(57,65)
(57,98)
(57,106)
(57,115)
(57,127)
(57,133)
(57,142)
(57,144)
(57,154)
(57,156)
(57,161)
(57,165)
(57,175)
(57,181)
(57,198)
(57,202)
(57,203)
(57,205)
(57,221)
(57,234)
(57,235)
(57,237)
(57,239)
(57,244)
(57,288)
(57,302)
(57,317)
(57,320)
(57,324)
(57,349)
(57,350)
(57,354)
(57,403)
(57,410)
(57,432)
(57,454)
(57,474)
(57,488)
(57,499)
(57,500)
(58,46)
(58,72)
(58,117)
(58,148)
(58,162)
(58,170)
(58,179)
(58,186)
(58,189)
(58,226)
(58,282)
(58,291)
(58,297)
(58,339)
(58,343)
(58,353)
(58,365)
(58,375)
(58,390)
(58,472)
(59,12)
(59,21)
(59,42)
(59,54)
(59,79)
(59,95)
(59,126)
(59,130)
(59,155)
(59,164)
(59,199)
(59,222)
(59,229)
(59,240)
(59,321)
(59,356)
(59,376)
(59,398)
(59,431)
(60,55)
(60,328)
(60,439)
(60,510)
(61,36)
(61,76)
(61,112)
(61,120)
(61,138)
(61,140)
(61,151)
(61,178)
(61,185)
(61,215)
(61,289)
(61,290)
(61,318)
(61,336)
(61,347)
(61,348)
(61,391)
(61,422)
(61,492)
(62,0)
(62,9)
(62,11)
(62,24)
(62,49)
(62,67)
(62,83)
(62,103)
(62,104)
(62,122)
(62,195)
(62,201)
(62,210)
(62,223)
(62,236)
(62,243)
(62,246)
(62,257)
(62,263)
(62,300)
(62,329)
(62,355)
(62,371)
(62,412)
(62,511)
(63,15)
(63,22)
(63,25)
(63,30)
(63,34)
(63,35)
(63,38)
(63,45)
(63,65)
(63,98)
(63,106)
(63,115)
(63,127)
(63,133)
(63,142)
(63,144)
(63,154)
(63,156)
(63,161)
(63,165)
(63,175)
(63,181)
(63,190)
(63,198)
(63,205)
(63,221)
(63,235)
(63,237)
(63,239)
(63,244)
(63,302)
(63,317)
(63,320)
(63,349)
(63,350)
(63,354)
(63,410)
(63,432)
(63,454)
(63,474)
(63,488)
(63,499)
(63,500)
(64,43)
(64,72)
(64,96)
(64,102)
(64,117)
(64,148)
(64,150)
(64,158)
(64,162)
(64,167)
(64,170)
(64,179)
(64,186)
(64,189)
(64,226)
(64,270)
(64,282)
(64,291)
(64,297)
(64,339)
(64,343)
(64,353)
(64,365)
(64,390)
(64,472)
(65,21)
(65,42)
(65,54)
(65,79)
(65,95)
(65,126)
(65,130)
(65,155)
(65,164)
(65,199)
(65,203)
(65,222)
(65,229)
(65,240)
(65,356)
(65,398)
(65,431)
(66,55)
(66,328)
(66,439)
(66,451)
(66,501)
(66,510)
(67,10)
(67,36)
(67,46)
(67,112)
(67,120)
(67,140)
(67,151)
(67,178)
(67,185)
(67,193)
(67,215)
(67,311)
(67,318)
(67,341)
(67,384)
(67,391)
(67,422)
(67,492)
(68,0)
(68,11)
(68,64)
(68,78)
(68,83)
(68,195)
(68,202)
(68,210)
(68,223)
(68,234)
(68,236)
(68,246)
(68,257)
(68,263)
(68,300)
(68,329)
(68,371)
(68,412)
(68,511)
(69,15)
(69,22)
(69,25)
(69,30)
(69,33)
(69,34)
(69,35)
(69,38)
(69,45)
(69,65)
(69,98)
(69,106)
(69,115)
(69,127)
(69,142)
(69,154)
(69,156)
(69,161)
(69,165)
(69,175)
(69,181)
(69,190)
(69,198)
(69,204)
(69,205)
(69,221)
(69,235)
(69,237)
(69,239)
(69,244)
(69,262)
(69,265)
(69,302)
(69,317)
(69,350)
(69,354)
(69,374)
(69,383)
(69,432)
(69,499)
(69,500)
(70,6)
(70,7)
(70,27)
(70,96)
(70,102)
(70,103)
(70,117)
(70,150)
(70,158)
(70,162)
(70,167)
(70,172)
(70,189)
(70,219)
(70,231)
(70,270)
(70,282)
(70,331)
(70,338)
(70,339)
(70,343)
(70,353)
(70,365)
(70,390)
(70,448)
(70,472)
(70,479)
(70,488)
(70,504)
(71,16)
(71,37)
(71,40)
(71,42)
(71,54)
(71,75)
(71,79)
(71,126)
(71,130)
(71,155)
(71,164)
(71,197)
(71,203)
(71,222)
(71,229)
(71,240)
(71,269)
(71,290)
(71,320)
(71,324)
(71,336)
(71,356)
(71,394)
(71,398)
(71,409)
(71,431)
(71,496)
(72,29)
(72,133)
(72,433)
(72,451)
(72,455)
(72,485)
(73,10)
(73,36)
(73,46)
(73,112)
(73,120)
(73,140)
(73,151)
(73,160)
(73,185)
(73,193)
(73,276)
(73,303)
(73,311)
(73,318)
(73,341)
(73,384)
(73,391)
(73,422)
(73,492)
(74,0)
(74,11)
(74,83)
(74,195)
(74,202)
(74,210)
(74,223)
(74,234)
(74,236)
(74,263)
(74,300)
(74,329)
(74,371)
(74,412)
(74,511)
(75,15)
(75,22)
(75,30)
(75,34)
(75,38)
(75,47)
(75,64)
(75,65)
(75,78)
(75,100)
(75,106)
(75,115)
(75,127)
(75,142)
(75,154)
(75,156)
(75,161)
(75,165)
(75,175)
(75,181)
(75,190)
(75,198)
(75,221)
(75,235)
(75,237)
(75,239)
(75,244)
(75,262)
(75,265)
(75,302)
(75,317)
(75,345)
(75,354)
(75,374)
(75,410)
(75,423)
(75,432)
(75,499)
(75,500)
(76,6)
(76,7)
(76,27)
(76,96)
(76,102)
(76,103)
(76,117)
(76,136)
(76,148)
(76,150)
(76,158)
(76,162)
(76,167)
(76,189)
(76,204)
(76,219)
(76,231)
(76,282)
(76,331)
(76,338)
(76,339)
(76,343)
(76,353)
(76,365)
(76,390)
(76,420)
(76,448)
(76,472)
(76,488)
(76,491)
(76,504)
(77,16)
(77,37)
(77,40)
(77,42)
(77,54)
(77,75)
(77,79)
(77,119)
(77,126)
(77,130)
(77,138)
(77,197)
(77,211)
(77,222)
(77,229)
(77,240)
(77,269)
(77,290)
(77,320)
(77,336)
(77,348)
(77,376)
(77,398)
(77,409)
(77,431)
(77,496)
(78,133)
(78,243)
(78,355)
(78,451)
(78,455)
(78,485)
(79,36)
(79,98)
(79,112)
(79,120)
(79,151)
(79,160)
(79,203)
(79,220)
(79,311)
(79,384)
(79,391)
(79,422)
(79,492)
(80,0)
(80,69)
(80,72)
(80,83)
(80,195)
(80,210)
(80,223)
(80,236)
(80,263)
(80,300)
(80,329)
(80,371)
(80,396)
(80,511)
(81,15)
(81,22)
(81,30)
(81,38)
(81,65)
(81,95)
(81,106)
(81,115)
(81,127)
(81,140)
(81,142)
(81,144)
(81,154)
(81,156)
(81,161)
(81,164)
(81,165)
(81,175)
(81,205)
(81,230)
(81,234)
(81,235)
(81,237)
(81,239)
(81,244)
(81,262)
(81,302)
(81,303)
(81,317)
(81,345)
(81,377)
(81,410)
(81,432)
(81,490)
(81,499)
(81,500)
(81,502)
(82,2)
(82,7)
(82,17)
(82,96)
(82,102)
(82,117)
(82,167)
(82,189)
(82,282)
(82,321)
(82,331)
(82,338)
(82,339)
(82,343)
(82,346)
(82,356)
(82,365)
(82,390)
(82,472)
(82,488)
(82,501)
(83,37)
(83,40)
(83,42)
(83,54)
(83,79)
(83,122)
(83,126)
(83,130)
(83,138)
(83,179)
(83,211)
(83,222)
(83,229)
(83,231)
(83,240)
(83,270)
(83,290)
(83,307)
(83,320)
(83,336)
(83,348)
(83,350)
(83,376)
(83,398)
(83,431)
(84,11)
(84,35)
(84,45)
(84,55)
(84,76)
(84,133)
(84,178)
(84,186)
(84,243)
(84,264)
(84,297)
(84,355)
(84,439)
(84,451)
(84,474)
(85,36)
(85,98)
(85,112)
(85,120)
(85,151)
(85,160)
(85,203)
(85,212)
(85,215)
(85,220)
(85,251)
(85,289)
(85,311)
(85,349)
(85,354)
(85,359)
(85,384)
(85,391)
(85,422)
(85,492)
(86,0)
(86,69)
(86,72)
(86,83)
(86,195)
(86,201)
(86,210)
(86,223)
(86,236)
(86,263)
(86,300)
(86,329)
(86,371)
(86,396)
(86,412)
(86,418)
(86,511)
(87,15)
(87,22)
(87,28)
(87,30)
(87,38)
(87,65)
(87,78)
(87,95)
(87,106)
(87,115)
(87,127)
(87,142)
(87,144)
(87,154)
(87,156)
(87,161)
(87,164)
(87,165)
(87,175)
(87,205)
(87,230)
(87,235)
(87,237)
(87,239)
(87,244)
(87,262)
(87,302)
(87,317)
(87,345)
(87,410)
(87,432)
(87,490)
(87,493)
(87,499)
(87,500)
(87,502)
(87,510)
(88,7)
(88,17)
(88,96)
(88,102)
(88,117)
(88,140)
(88,162)
(88,167)
(88,170)
(88,189)
(88,282)
(88,321)
(88,338)
(88,343)
(88,346)
(88,356)
(88,365)
(88,390)
(88,472)
(88,488)
(88,501)
(89,37)
(89,42)
(89,54)
(89,79)
(89,126)
(89,130)
(89,179)
(89,222)
(89,229)
(89,240)
(89,270)
(89,307)
(89,320)
(89,336)
(89,348)
(89,350)
(89,398)
(89,431)
(90,11)
(90,45)
(90,55)
(90,76)
(90,178)
(90,243)
(90,264)
(90,297)
(90,337)
(90,439)
(90,474)
(91,2)
(91,36)
(91,98)
(91,105)
(91,112)
(91,120)
(91,151)
(91,160)
(91,203)
(91,212)
(91,251)
(91,289)
(91,291)
(91,339)
(91,349)
(91,359)
(91,384)
(91,391)
(91,422)
(91,492)
(92,0)
(92,64)
(92,66)
(92,83)
(92,158)
(92,190)
(92,195)
(92,210)
(92,223)
(92,263)
(92,300)
(92,329)
(92,371)
(92,374)
(92,412)
(92,418)
(92,511)
(93,15)
(93,22)
(93,29)
(93,30)
(93,32)
(93,38)
(93,65)
(93,106)
(93,115)
(93,127)
(93,142)
(93,144)
(93,154)
(93,156)
(93,161)
(93,175)
(93,181)
(93,198)
(93,234)
(93,235)
(93,237)
(93,239)
(93,244)
(93,262)
(93,265)
(93,302)
(93,311)
(93,317)
(93,345)
(93,410)
(93,432)
(93,493)
(93,500)
(93,502)
(93,508)
(94,17)
(94,33)
(94,40)
(94,96)
(94,102)
(94,103)
(94,117)
(94,140)
(94,162)
(94,167)
(94,172)
(94,231)
(94,282)
(94,338)
(94,343)
(94,346)
(94,362)
(94,365)
(94,390)
(94,472)
(94,479)
(94,488)
(94,495)
(94,501)
(95,7)
(95,21)
(95,46)
(95,54)
(95,56)
(95,79)
(95,222)
(95,229)
(95,240)
(95,270)
(95,307)
(95,331)
(95,334)
(95,350)
(95,356)
(95,376)
(95,431)
(95,504)
(96,6)
(96,11)
(96,45)
(96,136)
(96,197)
(96,219)
(96,247)
(96,320)
(96,324)
(96,398)
(96,448)
(97,2)
(97,16)
(97,36)
(97,105)
(97,112)
(97,120)
(97,151)
(97,160)
(97,212)
(97,251)
(97,269)
(97,359)
(97,384)
(97,391)
(97,433)
(97,492)
(98,0)
(98,75)
(98,83)
(98,158)
(98,190)
(98,195)
(98,210)
(98,223)
(98,290)
(98,300)
(98,374)
(98,412)
(98,418)
(98,485)
(98,511)
(99,15)
(99,22)
(99,29)
(99,30)
(99,38)
(99,65)
(99,100)
(99,106)
(99,115)
(99,127)
(99,142)
(99,154)
(99,156)
(99,161)
(99,175)
(99,198)
(99,235)
(99,237)
(99,239)
(99,244)
(99,262)
(99,291)
(99,302)
(99,311)
(99,317)
(99,329)
(99,345)
(99,410)
(99,422)
(99,432)
(99,493)
(99,500)
(99,502)
(100,17)
(100,33)
(100,40)
(100,96)
(100,102)
(100,103)
(100,117)
(100,162)
(100,164)
(100,167)
(100,172)
(100,265)
(100,282)
(100,338)
(100,343)
(100,346)
(100,348)
(100,365)
(100,390)
(100,472)
(100,488)
(100,495)
(100,496)
(101,7)
(101,54)
(101,56)
(101,79)
(101,222)
(101,229)
(101,231)
(101,240)
(101,243)
(101,307)
(101,331)
(101,334)
(101,337)
(101,356)
(101,405)
(101,431)
(101,501)
(101,504)
(102,3)
(102,64)
(102,197)
(102,219)
(102,233)
(102,247)
(102,320)
(102,398)
(102,401)
(102,437)
(102,448)
(103,2)
(103,16)
(103,36)
(103,105)
(103,112)
(103,120)
(103,151)
(103,160)
(103,211)
(103,212)
(103,220)
(103,251)
(103,259)
(103,336)
(103,359)
(103,391)
(103,433)
(103,492)
(104,0)
(104,69)
(104,83)
(104,126)
(104,135)
(104,138)
(104,158)
(104,185)
(104,195)
(104,210)
(104,223)
(104,290)
(104,300)
(104,355)
(104,376)
(104,396)
(104,418)
(104,460)
(104,511)
(105,15)
(105,22)
(105,30)
(105,38)
(105,65)
(105,72)
(105,95)
(105,106)
(105,115)
(105,122)
(105,142)
(105,154)
(105,156)
(105,161)
(105,175)
(105,235)
(105,239)
(105,244)
(105,263)
(105,270)
(105,291)
(105,302)
(105,311)
(105,321)
(105,329)
(105,345)
(105,410)
(105,422)
(105,432)
(105,500)
(105,502)
(106,17)
(106,18)
(106,40)
(106,45)
(106,96)
(106,102)
(106,117)
(106,130)
(106,164)
(106,167)
(106,186)
(106,215)
(106,237)
(106,282)
(106,338)
(106,343)
(106,346)
(106,348)
(106,365)
(106,390)
(106,439)
(106,472)
(106,488)
(106,490)
(106,495)
(106,508)
(107,29)
(107,33)
(107,54)
(107,79)
(107,162)
(107,222)
(107,229)
(107,231)
(107,240)
(107,243)
(107,307)
(107,331)
(107,334)
(107,350)
(107,356)
(107,412)
(107,431)
(107,474)
(107,480)
(107,501)
(107,510)
(108,55)
(108,64)
(108,76)
(108,98)
(108,140)
(108,178)
(108,198)
(108,201)
(108,233)
(108,247)
(108,264)
(108,398)
(108,437)
(108,477)
(109,36)
(109,120)
(109,151)
(109,160)
(109,212)
(109,220)
(109,251)
(109,259)
(109,336)
(109,349)
(109,359)
(109,362)
(109,373)
(109,391)
(109,492)
(110,0)
(110,21)
(110,49)
(110,67)
(110,69)
(110,83)
(110,126)
(110,135)
(110,185)
(110,195)
(110,199)
(110,210)
(110,223)
(110,290)
(110,297)
(110,300)
(110,396)
(110,418)
(110,460)
(110,493)
(110,511)
(111,11)
(111,15)
(111,22)
(111,30)
(111,38)
(111,65)
(111,72)
(111,95)
(111,106)
(111,115)
(111,122)
(111,142)
(111,154)
(111,156)
(111,161)
(111,170)
(111,175)
(111,181)
(111,235)
(111,239)
(111,244)
(111,263)
(111,291)
(111,302)
(111,321)
(111,328)
(111,329)
(111,345)
(111,410)
(111,422)
(111,432)
(111,499)
(111,500)
(111,502)
(112,9)
(112,17)
(112,18)
(112,45)
(112,96)
(112,102)
(112,117)
(112,130)
(112,138)
(112,164)
(112,167)
(112,186)
(112,215)
(112,236)
(112,237)
(112,282)
(112,337)
(112,338)
(112,343)
(112,346)
(112,348)
(112,365)
(112,390)
(112,439)
(112,472)
(112,495)
(112,508)
(113,28)
(113,33)
(113,35)
(113,54)
(113,79)
(113,162)
(113,222)
(113,229)
(113,231)
(113,238)
(113,240)
(113,243)
(113,274)
(113,307)
(113,331)
(113,334)
(113,350)
(113,356)
(113,374)
(113,412)
(113,431)
(113,474)
(113,480)
(113,484)
(113,488)
(113,501)
(113,510)
(114,3)
(114,55)
(114,76)
(114,98)
(114,140)
(114,158)
(114,178)
(114,198)
(114,201)
(114,247)
(114,257)
(114,264)
(114,265)
(114,398)
(114,401)
(114,437)
(114,441)
(114,477)
(114,490)
(115,10)
(115,36)
(115,151)
(115,160)
(115,212)
(115,230)
(115,251)
(115,349)
(115,359)
(115,362)
(115,391)
(115,457)
(115,492)
(116,0)
(116,21)
(116,83)
(116,135)
(116,185)
(116,190)
(116,195)
(116,199)
(116,210)
(116,223)
(116,300)
(116,384)
(116,418)
(116,424)
(116,493)
(116,511)
(117,11)
(117,15)
(117,22)
(117,30)
(117,38)
(117,65)
(117,106)
(117,115)
(117,127)
(117,142)
(117,154)
(117,156)
(117,161)
(117,165)
(117,170)
(117,175)
(117,235)
(117,239)
(117,244)
(117,263)
(117,291)
(117,302)
(117,345)
(117,410)
(117,422)
(117,432)
(117,499)
(117,500)
(118,17)
(118,45)
(118,96)
(118,102)
(118,117)
(118,130)
(118,164)
(118,167)
(118,219)
(118,236)
(118,282)
(118,337)
(118,338)
(118,343)
(118,346)
(118,365)
(118,390)
(118,439)
(118,472)
(118,479)
(118,495)
(118,508)
(119,6)
(119,33)
(119,54)
(119,56)
(119,75)
(119,79)
(119,112)
(119,144)
(119,162)
(119,222)
(119,229)
(119,231)
(119,232)
(119,238)
(119,240)
(119,243)
(119,269)
(119,274)
(119,307)
(119,331)
(119,334)
(119,335)
(119,350)
(119,356)
(119,374)
(119,412)
(119,431)
(119,448)
(119,488)
(119,501)
(119,504)
(120,2)
(120,3)
(120,16)
(120,29)
(120,40)
(120,98)
(120,140)
(120,158)
(120,197)
(120,247)
(120,257)
(120,265)
(120,278)
(120,290)
(120,320)
(120,401)
(120,420)
(120,437)
(120,441)
(120,485)
(121,36)
(121,151)
(121,160)
(121,212)
(121,230)
(121,251)
(121,270)
(121,329)
(121,359)
(121,376)
(121,391)
(121,457)
(121,492)
(122,0)
(122,21)
(122,83)
(122,135)
(122,185)
(122,190)
(122,195)
(122,199)
(122,210)
(122,223)
(122,300)
(122,398)
(122,416)
(122,418)
(122,424)
(122,433)
(122,511)
(123,15)
(123,22)
(123,30)
(123,38)
(123,65)
(123,100)
(123,106)
(123,115)
(123,142)
(123,154)
(123,156)
(123,161)
(123,165)
(123,235)
(123,239)
(123,244)
(123,263)
(123,291)
(123,302)
(123,345)
(123,362)
(123,405)
(123,410)
(123,422)
(123,432)
(123,499)
(123,500)
(124,17)
(124,63)
(124,96)
(124,102)
(124,117)
(124,130)
(124,164)
(124,167)
(124,219)
(124,236)
(124,282)
(124,337)
(124,338)
(124,343)
(124,346)
(124,365)
(124,472)
(124,495)
(124,508)
(125,6)
(125,33)
(125,54)
(125,56)
(125,75)
(125,79)
(125,112)
(125,162)
(125,229)
(125,231)
(125,232)
(125,238)
(125,240)
(125,243)
(125,269)
(125,274)
(125,307)
(125,331)
(125,334)
(125,335)
(125,367)
(125,412)
(125,431)
(125,448)
(125,501)
(125,504)
(126,2)
(126,3)
(126,16)
(126,29)
(126,40)
(126,103)
(126,105)
(126,136)
(126,138)
(126,140)
(126,158)
(126,197)
(126,198)
(126,211)
(126,247)
(126,257)
(126,259)
(126,265)
(126,278)
(126,290)
(126,305)
(126,320)
(126,356)
(126,401)
(126,437)
(126,441)
(126,485)
(127,18)
(127,46)
(127,64)
(127,69)
(127,122)
(127,151)
(127,160)
(127,212)
(127,230)
(127,251)
(127,329)
(127,336)
(127,359)
(127,376)
(127,390)
(127,391)
(127,492)
(127,506)
(128,21)
(128,83)
(128,135)
(128,195)
(128,199)
(128,210)
(128,223)
(128,233)
(128,264)
(128,300)
(128,396)
(128,398)
(128,418)
(128,511)
(129,0)
(129,15)
(129,22)
(129,30)
(129,38)
(129,65)
(129,68)
(129,106)
(129,115)
(129,126)
(129,142)
(129,154)
(129,156)
(129,161)
(129,186)
(129,235)
(129,239)
(129,244)
(129,291)
(129,302)
(129,345)
(129,355)
(129,410)
(129,422)
(129,432)
(129,500)
(130,17)
(130,72)
(130,95)
(130,96)
(130,102)
(130,117)
(130,130)
(130,164)
(130,167)
(130,282)
(130,321)
(130,338)
(130,343)
(130,346)
(130,365)
(130,460)
(130,472)
(130,495)
(130,508)
(131,33)
(131,45)
(131,54)
(131,79)
(131,112)
(131,120)
(131,162)
(131,229)
(131,231)
(131,238)
(131,240)
(131,243)
(131,274)
(131,307)
(131,331)
(131,335)
(131,350)
(131,412)
(131,431)
(132,2)
(132,3)
(132,40)
(132,55)
(132,105)
(132,138)
(132,158)
(132,198)
(132,211)
(132,247)
(132,257)
(132,259)
(132,290)
(132,305)
(132,320)
(132,356)
(132,401)
(132,437)
(132,439)
(132,441)
(132,485)
(133,18)
(133,35)
(133,64)
(133,67)
(133,69)
(133,76)
(133,122)
(133,160)
(133,178)
(133,201)
(133,202)
(133,212)
(133,215)
(133,230)
(133,251)
(133,277)
(133,297)
(133,329)
(133,336)
(133,349)
(133,359)
(133,373)
(133,391)
(133,474)
(133,492)
(133,493)
(133,499)
(133,501)
(133,502)
(133,506)
(133,510)
(134,9)
(134,11)
(134,21)
(134,28)
(134,49)
(134,135)
(134,140)
(134,151)
(134,170)
(134,185)
(134,195)
(134,199)
(134,210)
(134,223)
(134,263)
(134,264)
(134,300)
(134,337)
(134,390)
(134,396)
(134,398)
(134,418)
(134,451)
(134,477)
(134,490)
(134,511)
(135,0)
(135,15)
(135,22)
(135,30)
(135,38)
(135,44)
(135,46)
(135,65)
(135,68)
(135,106)
(135,115)
(135,126)
(135,142)
(135,154)
(135,156)
(135,161)
(135,186)
(135,235)
(135,239)
(135,244)
(135,291)
(135,302)
(135,345)
(135,410)
(135,422)
(135,432)
(135,500)
(136,17)
(136,95)
(136,96)
(136,102)
(136,117)
(136,130)
(136,164)
(136,167)
(136,282)
(136,321)
(136,338)
(136,343)
(136,346)
(136,365)
(136,472)
(136,495)
(136,508)
(137,33)
(137,45)
(137,54)
(137,79)
(137,83)
(137,112)
(137,162)
(137,229)
(137,231)
(137,238)
(137,240)
(137,270)
(137,274)
(137,307)
(137,331)
(137,335)
(137,350)
(137,412)
(137,431)
(137,460)
(138,55)
(138,105)
(138,158)
(138,198)
(138,236)
(138,247)
(138,257)
(138,305)
(138,401)
(138,439)
(138,441)
(138,457)
(138,485)
(139,18)
(139,35)
(139,127)
(139,160)
(139,178)
(139,201)
(139,212)
(139,215)
(139,230)
(139,251)
(139,265)
(139,297)
(139,329)
(139,349)
(139,359)
(139,372)
(139,391)
(139,437)
(139,474)
(139,492)
(139,493)
(139,499)
(139,501)
(139,506)
(140,9)
(140,10)
(140,11)
(140,21)
(140,64)
(140,135)
(140,136)
(140,140)
(140,170)
(140,185)
(140,195)
(140,199)
(140,205)
(140,210)
(140,223)
(140,264)
(140,300)
(140,374)
(140,384)
(140,390)
(140,398)
(140,418)
(140,511)
(141,0)
(141,15)
(141,22)
(141,27)
(141,30)
(141,38)
(141,65)
(141,68)
(141,106)
(141,115)
(141,154)
(141,161)
(141,190)
(141,235)
(141,239)
(141,244)
(141,291)
(141,302)
(141,345)
(141,367)
(141,410)
(141,422)
(141,432)
(141,461)
(141,500)
(142,17)
(142,40)
(142,95)
(142,96)
(142,102)
(142,117)
(142,164)
(142,167)
(142,219)
(142,234)
(142,262)
(142,282)
(142,334)
(142,343)
(142,346)
(142,365)
(142,472)
(142,479)
(142,495)
(142,504)
(142,508)
(143,2)
(143,33)
(143,45)
(143,46)
(143,54)
(143,56)
(143,75)
(143,79)
(143,83)
(143,112)
(143,162)
(143,222)
(143,229)
(143,231)
(143,233)
(143,238)
(143,240)
(143,274)
(143,307)
(143,331)
(143,335)
(143,338)
(143,356)
(143,412)
(143,431)
(143,460)
(144,16)
(144,63)
(144,158)
(144,198)
(144,236)
(144,247)
(144,257)
(144,305)
(144,401)
(144,416)
(144,433)
(144,441)
(144,457)
(144,485)
(145,6)
(145,7)
(145,18)
(145,127)
(145,160)
(145,189)
(145,197)
(145,212)
(145,230)
(145,251)
(145,265)
(145,269)
(145,290)
(145,320)
(145,329)
(145,359)
(145,372)
(145,391)
(145,437)
(145,448)
(145,492)
(145,493)
(145,499)
(145,501)
(145,506)
(146,11)
(146,21)
(146,135)
(146,136)
(146,140)
(146,195)
(146,210)
(146,223)
(146,300)
(146,374)
(146,376)
(146,398)
(146,418)
(146,511)
(147,15)
(147,22)
(147,27)
(147,30)
(147,38)
(147,65)
(147,100)
(147,106)
(147,115)
(147,154)
(147,161)
(147,205)
(147,235)
(147,239)
(147,244)
(147,255)
(147,291)
(147,302)
(147,345)
(147,367)
(147,410)
(147,422)
(147,423)
(147,432)
(147,500)
(148,17)
(148,40)
(148,95)
(148,96)
(148,102)
(148,117)
(148,164)
(148,167)
(148,219)
(148,262)
(148,282)
(148,334)
(148,337)
(148,343)
(148,346)
(148,365)
(148,461)
(148,472)
(148,479)
(148,495)
(148,504)
(148,508)
(149,2)
(149,33)
(149,54)
(149,56)
(149,75)
(149,79)
(149,83)
(149,112)
(149,156)
(149,162)
(149,222)
(149,229)
(149,231)
(149,233)
(149,238)
(149,240)
(149,259)
(149,274)
(149,307)
(149,331)
(149,335)
(149,338)
(149,356)
(149,405)
(149,412)
(149,431)
(149,460)
(150,16)
(150,46)
(150,63)
(150,138)
(150,158)
(150,198)
(150,247)
(150,257)
(150,305)
(150,401)
(150,416)
(150,420)
(150,433)
(150,441)
(150,457)
(150,485)
(150,496)
(151,7)
(151,18)
(151,103)
(151,142)
(151,151)
(151,159)
(151,189)
(151,197)
(151,211)
(151,212)
(151,230)
(151,251)
(151,265)
(151,290)
(151,320)
(151,329)
(151,359)
(151,391)
(151,396)
(151,437)
(151,492)
(151,499)
(151,506)
(152,135)
(152,173)
(152,195)
(152,210)
(152,223)
(152,232)
(152,300)
(152,362)
(152,398)
(152,418)
(152,493)
(152,511)
(153,15)
(153,22)
(153,30)
(153,38)
(153,65)
(153,106)
(153,115)
(153,154)
(153,161)
(153,165)
(153,235)
(153,239)
(153,244)
(153,291)
(153,302)
(153,345)
(153,367)
(153,410)
(153,422)
(153,500)
(154,17)
(154,40)
(154,72)
(154,95)
(154,96)
(154,102)
(154,117)
(154,164)
(154,167)
(154,186)
(154,282)
(154,334)
(154,343)
(154,346)
(154,350)
(154,365)
(154,472)
(154,495)
(154,508)
(155,33)
(155,79)
(155,120)
(155,122)
(155,126)
(155,130)
(155,156)
(155,162)
(155,193)
(155,199)
(155,229)
(155,231)
(155,240)
(155,259)
(155,274)
(155,307)
(155,311)
(155,321)
(155,331)
(155,335)
(155,338)
(155,356)
(155,412)
(155,431)
(155,439)
(155,501)
(156,28)
(156,29)
(156,35)
(156,55)
(156,63)
(156,68)
(156,76)
(156,138)
(156,198)
(156,201)
(156,202)
(156,238)
(156,247)
(156,257)
(156,264)
(156,297)
(156,349)
(156,401)
(156,416)
(156,441)
(156,485)
(157,3)
(157,7)
(157,18)
(157,45)
(157,69)
(157,151)
(157,158)
(157,159)
(157,178)
(157,189)
(157,211)
(157,212)
(157,251)
(157,277)
(157,290)
(157,305)
(157,320)
(157,329)
(157,359)
(157,372)
(157,373)
(157,387)
(157,391)
(157,396)
(157,407)
(157,437)
(157,474)
(157,492)
(157,499)
(157,506)
(158,9)
(158,21)
(158,83)
(158,135)
(158,140)
(158,142)
(158,144)
(158,170)
(158,173)
(158,195)
(158,210)
(158,215)
(158,223)
(158,230)
(158,270)
(158,300)
(158,398)
(158,418)
(158,427)
(158,493)
(158,510)
(159,15)
(159,22)
(159,30)
(159,38)
(159,65)
(159,106)
(159,115)
(159,154)
(159,161)
(159,165)
(159,239)
(159,244)
(159,291)
(159,302)
(159,337)
(159,345)
(159,410)
(159,422)
(159,500)
(160,17)
(160,40)
(160,95)
(160,96)
(160,102)
(160,117)
(160,164)
(160,167)
(160,186)
(160,282)
(160,334)
(160,343)
(160,346)
(160,350)
(160,365)
(160,472)
(160,495)
(160,508)
(161,0)
(161,33)
(161,79)
(161,113)
(161,130)
(161,156)
(161,162)
(161,199)
(161,229)
(161,240)
(161,274)
(161,307)
(161,314)
(161,331)
(161,335)
(161,338)
(161,367)
(161,412)
(161,431)
(161,439)
(161,501)
(162,35)
(162,55)
(162,68)
(162,76)
(162,198)
(162,201)
(162,231)
(162,238)
(162,247)
(162,257)
(162,264)
(162,297)
(162,349)
(162,356)
(162,401)
(162,416)
(162,441)
(162,485)
(163,7)
(163,11)
(163,18)
(163,46)
(163,136)
(163,158)
(163,159)
(163,178)
(163,189)
(163,212)
(163,236)
(163,251)
(163,265)
(163,305)
(163,329)
(163,359)
(163,387)
(163,391)
(163,407)
(163,437)
(163,457)
(163,474)
(163,492)
(163,499)
(163,506)
(164,5)
(164,12)
(164,21)
(164,63)
(164,83)
(164,112)
(164,135)
(164,140)
(164,142)
(164,170)
(164,173)
(164,195)
(164,210)
(164,223)
(164,230)
(164,232)
(164,300)
(164,372)
(164,374)
(164,390)
(164,398)
(164,418)
(164,427)
(164,488)
(164,511)
(165,15)
(165,22)
(165,30)
(165,38)
(165,65)
(165,106)
(165,115)
(165,154)
(165,161)
(165,165)
(165,239)
(165,244)
(165,270)
(165,291)
(165,302)
(165,345)
(165,422)
(165,479)
(165,500)
(166,17)
(166,27)
(166,40)
(166,96)
(166,102)
(166,117)
(166,164)
(166,167)
(166,233)
(166,282)
(166,334)
(166,343)
(166,346)
(166,350)
(166,365)
(166,384)
(166,461)
(166,472)
(166,495)
(166,508)
(167,0)
(167,6)
(167,33)
(167,79)
(167,113)
(167,156)
(167,160)
(167,162)
(167,199)
(167,219)
(167,222)
(167,229)
(167,240)
(167,274)
(167,307)
(167,314)
(167,331)
(167,335)
(167,337)
(167,338)
(167,367)
(167,412)
(167,431)
(167,447)
(167,501)
(167,504)
(168,2)
(168,3)
(168,16)
(168,56)
(168,75)
(168,105)
(168,198)
(168,231)
(168,238)
(168,247)
(168,257)
(168,264)
(168,269)
(168,290)
(168,356)
(168,401)
(168,416)
(168,441)
(168,485)
(169,7)
(169,11)
(169,18)
(169,46)
(169,136)
(169,158)
(169,159)
(169,189)
(169,212)
(169,251)
(169,265)
(169,305)
(169,320)
(169,329)
(169,359)
(169,387)
(169,391)
(169,407)
(169,437)
(169,457)
(169,492)
(169,499)
(169,506)
(170,12)
(170,21)
(170,63)
(170,83)
(170,112)
(170,135)
(170,140)
(170,142)
(170,195)
(170,205)
(170,210)
(170,223)
(170,232)
(170,236)
(170,300)
(170,372)
(170,423)
(170,427)
(170,488)
(170,511)
(171,15)
(171,22)
(171,30)
(171,38)
(171,65)
(171,106)
(171,115)
(171,154)
(171,161)
(171,165)
(171,239)
(171,244)
(171,291)
(171,302)
(171,345)
(171,374)
(171,410)
(171,422)
(171,432)
(171,448)
(171,500)
(172,17)
(172,27)
(172,40)
(172,96)
(172,100)
(172,102)
(172,117)
(172,164)
(172,167)
(172,197)
(172,233)
(172,282)
(172,334)
(172,343)
(172,346)
(172,365)
(172,472)
(172,479)
(172,495)
(172,508)
(173,33)
(173,79)
(173,113)
(173,156)
(173,160)
(173,162)
(173,219)
(173,222)
(173,229)
(173,240)
(173,274)
(173,307)
(173,331)
(173,335)
(173,338)
(173,367)
(173,412)
(173,418)
(173,431)
(173,447)
(173,501)
(173,504)
(174,2)
(174,16)
(174,56)
(174,75)
(174,231)
(174,238)
(174,247)
(174,257)
(174,259)
(174,269)
(174,290)
(174,314)
(174,356)
(174,384)
(174,398)
(174,401)
(174,416)
(174,433)
(174,441)
(174,485)
(175,3)
(175,7)
(175,18)
(175,46)
(175,68)
(175,136)
(175,138)
(175,158)
(175,159)
(175,172)
(175,189)
(175,212)
(175,251)
(175,305)
(175,320)
(175,329)
(175,359)
(175,387)
(175,391)
(175,437)
(175,457)
(175,492)
(175,506)
(176,12)
(176,63)
(176,64)
(176,69)
(176,83)
(176,95)
(176,112)
(176,135)
(176,148)
(176,195)
(176,210)
(176,211)
(176,223)
(176,300)
(176,427)
(176,509)
(176,511)
(177,15)
(177,22)
(177,30)
(177,38)
(177,65)
(177,106)
(177,115)
(177,130)
(177,154)
(177,161)
(177,165)
(177,239)
(177,244)
(177,291)
(177,302)
(177,345)
(177,350)
(177,410)
(177,422)
(177,500)
(178,17)
(178,35)
(178,40)
(178,72)
(178,96)
(178,102)
(178,117)
(178,120)
(178,122)
(178,164)
(178,167)
(178,201)
(178,233)
(178,277)
(178,282)
(178,334)
(178,343)
(178,346)
(178,365)
(178,472)
(178,479)
(178,495)
(178,508)
(179,29)
(179,33)
(179,79)
(179,113)
(179,126)
(179,144)
(179,156)
(179,160)
(179,162)
(179,186)
(179,222)
(179,229)
(179,240)
(179,274)
(179,307)
(179,311)
(179,321)
(179,331)
(179,335)
(179,338)
(179,349)
(179,367)
(179,396)
(179,412)
(179,418)
(179,431)
(179,447)
(179,501)
(180,2)
(180,55)
(180,76)
(180,151)
(180,231)
(180,238)
(180,247)
(180,257)
(180,259)
(180,264)
(180,290)
(180,297)
(180,314)
(180,356)
(180,372)
(180,373)
(180,384)
(180,398)
(180,401)
(180,439)
(180,441)
(180,499)
(181,3)
(181,7)
(181,18)
(181,28)
(181,46)
(181,68)
(181,136)
(181,138)
(181,158)
(181,159)
(181,172)
(181,189)
(181,215)
(181,251)
(181,305)
(181,320)
(181,329)
(181,337)
(181,359)
(181,387)
(181,391)
(181,416)
(181,437)
(181,474)
(181,492)
(181,506)
(182,5)
(182,9)
(182,12)
(182,49)
(182,64)
(182,69)
(182,83)
(182,95)
(182,112)
(182,135)
(182,170)
(182,195)
(182,198)
(182,210)
(182,223)
(182,300)
(182,427)
(182,457)
(182,477)
(182,493)
(182,509)
(182,510)
(182,511)
(183,15)
(183,21)
(183,22)
(183,30)
(183,38)
(183,65)
(183,106)
(183,115)
(183,130)
(183,140)
(183,154)
(183,161)
(183,165)
(183,239)
(183,244)
(183,263)
(183,291)
(183,302)
(183,345)
(183,350)
(183,410)
(183,422)
(183,500)
(184,17)
(184,35)
(184,96)
(184,102)
(184,117)
(184,120)
(184,164)
(184,167)
(184,201)
(184,277)
(184,282)
(184,334)
(184,343)
(184,346)
(184,365)
(184,451)
(184,472)
(184,479)
(184,495)
(184,508)
(185,33)
(185,40)
(185,79)
(185,113)
(185,156)
(185,160)
(185,162)
(185,186)
(185,212)
(185,222)
(185,229)
(185,230)
(185,233)
(185,240)
(185,274)
(185,307)
(185,331)
(185,335)
(185,338)
(185,349)
(185,367)
(185,412)
(185,418)
(185,431)
(185,447)
(185,501)
(186,55)
(186,205)
(186,238)
(186,247)
(186,257)
(186,264)
(186,265)
(186,290)
(186,297)
(186,311)
(186,314)
(186,372)
(186,373)
(186,384)
(186,398)
(186,401)
(186,439)
(186,441)
(186,499)
(187,0)
(187,7)
(187,18)
(187,46)
(187,136)
(187,144)
(187,148)
(187,158)
(187,159)
(187,172)
(187,175)
(187,189)
(187,206)
(187,251)
(187,305)
(187,329)
(187,359)
(187,387)
(187,391)
(187,416)
(187,437)
(187,492)
(187,506)
(188,9)
(188,11)
(188,12)
(188,54)
(188,95)
(188,105)
(188,112)
(188,135)
(188,170)
(188,195)
(188,198)
(188,210)
(188,223)
(188,236)
(188,300)
(188,354)
(188,427)
(188,493)
(188,509)
(189,15)
(189,21)
(189,22)
(189,27)
(189,30)
(189,38)
(189,65)
(189,85)
(189,106)
(189,115)
(189,130)
(189,154)
(189,161)
(189,165)
(189,239)
(189,244)
(189,291)
(189,302)
(189,345)
(189,350)
(189,374)
(189,422)
(189,461)
(190,10)
(190,17)
(190,96)
(190,102)
(190,117)
(190,140)
(190,164)
(190,167)
(190,231)
(190,232)
(190,270)
(190,282)
(190,334)
(190,343)
(190,346)
(190,363)
(190,365)
(190,472)
(190,479)
(190,488)
(190,495)
(190,508)
(191,6)
(191,33)
(191,40)
(191,63)
(191,75)
(191,79)
(191,113)
(191,156)
(191,160)
(191,162)
(191,212)
(191,222)
(191,229)
(191,240)
(191,243)
(191,274)
(191,307)
(191,320)
(191,330)
(191,331)
(191,335)
(191,338)
(191,367)
(191,412)
(191,418)
(191,431)
(191,438)
(191,447)
(191,485)
(191,501)
(191,504)
(192,2)
(192,16)
(192,56)
(192,233)
(192,238)
(192,247)
(192,257)
(192,265)
(192,290)
(192,311)
(192,314)
(192,384)
(192,398)
(192,401)
(192,433)
(192,441)
(192,499)
(193,0)
(193,7)
(193,18)
(193,46)
(193,100)
(193,136)
(193,148)
(193,158)
(193,159)
(193,172)
(193,189)
(193,197)
(193,205)
(193,206)
(193,251)
(193,305)
(193,329)
(193,337)
(193,359)
(193,372)
(193,373)
(193,387)
(193,391)
(193,416)
(193,437)
(193,492)
(193,506)
(194,11)
(194,12)
(194,54)
(194,80)
(194,82)
(194,103)
(194,105)
(194,112)
(194,135)
(194,144)
(194,175)
(194,183)
(194,195)
(194,198)
(194,210)
(194,223)
(194,300)
(194,356)
(194,427)
(194,493)
(194,509)
(195,15)
(195,21)
(195,22)
(195,27)
(195,30)
(195,38)
(195,48)
(195,65)
(195,69)
(195,85)
(195,106)
(195,115)
(195,130)
(195,154)
(195,161)
(195,165)
(195,230)
(195,236)
(195,239)
(195,244)
(195,269)
(195,291)
(195,302)
(195,345)
(195,410)
(195,422)
(195,461)
(196,17)
(196,96)
(196,102)
(196,117)
(196,140)
(196,164)
(196,167)
(196,231)
(196,232)
(196,282)
(196,334)
(196,343)
(196,346)
(196,365)
(196,374)
(196,413)
(196,423)
(196,457)
(196,472)
(196,479)
(196,488)
(196,495)
(196,500)
(197,6)
(197,33)
(197,40)
(197,63)
(197,75)
(197,79)
(197,113)
(197,156)
(197,160)
(197,162)
(197,212)
(197,222)
(197,229)
(197,240)
(197,270)
(197,274)
(197,307)
(197,320)
(197,331)
(197,335)
(197,338)
(197,363)
(197,367)
(197,405)
(197,412)
(197,418)
(197,431)
(197,447)
(197,448)
(197,485)
(197,501)
(197,504)
(198,2)
(198,16)
(198,56)
(198,151)
(198,211)
(198,233)
(198,238)
(198,247)
(198,257)
(198,259)
(198,265)
(198,267)
(198,290)
(198,311)
(198,314)
(198,354)
(198,398)
(198,401)
(198,433)
(198,441)
(198,469)
(198,496)
(198,499)
(199,7)
(199,18)
(199,46)
(199,148)
(199,158)
(199,159)
(199,172)
(199,189)
(199,197)
(199,206)
(199,251)
(199,305)
(199,324)
(199,329)
(199,359)
(199,387)
(199,391)
(199,396)
(199,407)
(199,416)
(199,437)
(199,492)
(199,506)
(199,511)
(200,12)
(200,42)
(200,54)
(200,80)
(200,112)
(200,114)
(200,135)
(200,138)
(200,175)
(200,183)
(200,195)
(200,223)
(200,300)
(200,427)
(200,509)
(201,15)
(201,22)
(201,30)
(201,38)
(201,48)
(201,65)
(201,69)
(201,104)
(201,106)
(201,115)
(201,122)
(201,126)
(201,130)
(201,154)
(201,161)
(201,165)
(201,230)
(201,239)
(201,244)
(201,291)
(201,302)
(201,321)
(201,345)
(201,355)
(201,410)
(201,422)
(202,17)
(202,72)
(202,96)
(202,102)
(202,117)
(202,120)
(202,164)
(202,167)
(202,186)
(202,232)
(202,282)
(202,330)
(202,334)
(202,343)
(202,346)
(202,365)
(202,369)
(202,413)
(202,457)
(202,472)
(202,495)
(202,500)
(203,33)
(203,63)
(203,79)
(203,95)
(203,107)
(203,113)
(203,156)
(203,160)
(203,162)
(203,212)
(203,229)
(203,240)
(203,274)
(203,307)
(203,320)
(203,331)
(203,335)
(203,338)
(203,367)
(203,412)
(203,418)
(203,431)
(203,447)
(203,474)
(203,480)
(203,485)
(203,501)
(203,502)
(204,76)
(204,82)
(204,211)
(204,233)
(204,238)
(204,247)
(204,257)
(204,259)
(204,290)
(204,297)
(204,314)
(204,350)
(204,354)
(204,398)
(204,401)
(204,441)
(204,499)
(205,5)
(205,7)
(205,18)
(205,46)
(205,55)
(205,67)
(205,68)
(205,148)
(205,151)
(205,158)
(205,159)
(205,172)
(205,178)
(205,189)
(205,201)
(205,205)
(205,206)
(205,215)
(205,251)
(205,268)
(205,277)
(205,289)
(205,305)
(205,329)
(205,337)
(205,349)
(205,359)
(205,373)
(205,376)
(205,387)
(205,391)
(205,396)
(205,407)
(205,416)
(205,437)
(205,439)
(205,490)
(205,492)
(205,506)
(205,511)
(206,9)
(206,12)
(206,19)
(206,35)
(206,49)
(206,54)
(206,80)
(206,85)
(206,112)
(206,114)
(206,135)
(206,138)
(206,170)
(206,175)
(206,183)
(206,195)
(206,198)
(206,199)
(206,210)
(206,223)
(206,300)
(206,353)
(206,427)
(206,509)
(207,15)
(207,22)
(207,30)
(207,38)
(207,48)
(207,65)
(207,69)
(207,104)
(207,106)
(207,115)
(207,122)
(207,126)
(207,130)
(207,154)
(207,161)
(207,165)
(207,230)
(207,239)
(207,244)
(207,291)
(207,302)
(207,321)
(207,345)
(207,356)
(207,363)
(207,410)
(207,422)
(208,17)
(208,72)
(208,96)
(208,102)
(208,117)
(208,120)
(208,164)
(208,167)
(208,186)
(208,270)
(208,282)
(208,317)
(208,330)
(208,334)
(208,343)
(208,346)
(208,365)
(208,369)
(208,413)
(208,457)
(208,495)
(208,500)
(208,510)
(209,11)
(209,33)
(209,79)
(209,95)
(209,107)
(209,113)
(209,144)
(209,156)
(209,160)
(209,162)
(209,229)
(209,231)
(209,237)
(209,240)
(209,263)
(209,274)
(209,280)
(209,307)
(209,320)
(209,335)
(209,338)
(209,367)
(209,412)
(209,418)
(209,431)
(209,447)
(209,472)
(209,474)
(209,480)
(209,485)
(209,493)
(209,501)
(210,10)
(210,76)
(210,82)
(210,236)
(210,238)
(210,247)
(210,257)
(210,265)
(210,297)
(210,314)
(210,350)
(210,354)
(210,398)
(210,401)
(210,441)
(210,477)
(210,499)
(211,7)
(211,46)
(211,105)
(211,140)
(211,148)
(211,159)
(211,172)
(211,178)
(211,189)
(211,205)
(211,251)
(211,289)
(211,305)
(211,329)
(211,349)
(211,359)
(211,376)
(211,387)
(211,391)
(211,416)
(211,437)
(211,439)
(211,492)
(211,506)
(211,511)
(212,19)
(212,54)
(212,80)
(212,112)
(212,135)
(212,170)
(212,175)
(212,183)
(212,190)
(212,195)
(212,198)
(212,222)
(212,223)
(212,300)
(212,353)
(212,427)
(212,509)
(213,15)
(213,22)
(213,30)
(213,38)
(213,48)
(213,65)
(213,69)
(213,104)
(213,106)
(213,115)
(213,134)
(213,154)
(213,161)
(213,165)
(213,230)
(213,239)
(213,244)
(213,291)
(213,302)
(213,321)
(213,345)
(213,363)
(213,372)
(213,384)
(213,410)
(213,422)
(213,479)
(214,17)
(214,96)
(214,102)
(214,117)
(214,164)
(214,167)
(214,210)
(214,270)
(214,282)
(214,317)
(214,330)
(214,334)
(214,343)
(214,346)
(214,357)
(214,365)
(214,369)
(214,413)
(214,495)
(215,11)
(215,27)
(215,33)
(215,78)
(215,79)
(215,95)
(215,107)
(215,113)
(215,156)
(215,160)
(215,162)
(215,229)
(215,231)
(215,237)
(215,240)
(215,274)
(215,280)
(215,307)
(215,324)
(215,335)
(215,338)
(215,367)
(215,374)
(215,412)
(215,418)
(215,431)
(215,472)
(215,485)
(215,501)
(215,508)
(216,6)
(216,56)
(216,58)
(216,82)
(216,219)
(216,236)
(216,238)
(216,247)
(216,265)
(216,269)
(216,350)
(216,398)
(216,401)
(216,441)
(216,488)
(216,504)
(217,7)
(217,16)
(217,46)
(217,63)
(217,75)
(217,100)
(217,105)
(217,148)
(217,158)
(217,159)
(217,172)
(217,189)
(217,251)
(217,257)
(217,262)
(217,289)
(217,290)
(217,305)
(217,320)
(217,359)
(217,376)
(217,387)
(217,391)
(217,416)
(217,437)
(217,448)
(217,469)
(217,492)
(217,506)
(218,10)
(218,19)
(218,54)
(218,80)
(218,112)
(218,135)
(218,170)
(218,175)
(218,183)
(218,190)
(218,195)
(218,197)
(218,198)
(218,222)
(218,223)
(218,300)
(218,405)
(218,427)
(218,447)
(218,509)
(219,15)
(219,22)
(219,30)
(219,38)
(219,47)
(219,48)
(219,65)
(219,69)
(219,104)
(219,106)
(219,115)
(219,134)
(219,154)
(219,165)
(219,239)
(219,244)
(219,291)
(219,302)
(219,321)
(219,345)
(219,353)
(219,363)
(219,404)
(219,410)
(219,420)
(219,422)
(219,433)
(219,479)
(219,496)
(220,17)
(220,96)
(220,102)
(220,117)
(220,164)
(220,167)
(220,210)
(220,270)
(220,282)
(220,330)
(220,334)
(220,343)
(220,346)
(220,357)
(220,365)
(220,369)
(220,413)
(220,423)
(220,495)
(221,27)
(221,33)
(221,61)
(221,79)
(221,113)
(221,156)
(221,160)
(221,162)
(221,229)
(221,231)
(221,240)
(221,274)
(221,307)
(221,335)
(221,337)
(221,338)
(221,367)
(221,412)
(221,418)
(221,431)
(221,472)
(221,485)
(222,6)
(222,40)
(222,56)
(222,82)
(222,99)
(222,219)
(222,233)
(222,238)
(222,247)
(222,263)
(222,265)
(222,269)
(222,317)
(222,398)
(222,401)
(222,441)
(222,488)
(222,504)
(223,7)
(223,16)
(223,46)
(223,63)
(223,100)
(223,103)
(223,105)
(223,138)
(223,148)
(223,158)
(223,159)
(223,172)
(223,189)
(223,208)
(223,211)
(223,251)
(223,257)
(223,262)
(223,289)
(223,290)
(223,305)
(223,320)
(223,324)
(223,336)
(223,359)
(223,376)
(223,387)
(223,391)
(223,416)
(223,437)
(223,457)
(223,469)
(223,492)
(223,506)
(224,10)
(224,19)
(224,54)
(224,68)
(224,72)
(224,80)
(224,95)
(224,112)
(224,122)
(224,126)
(224,135)
(224,175)
(224,183)
(224,195)
(224,198)
(224,212)
(224,222)
(224,223)
(224,230)
(224,259)
(224,280)
(224,300)
(224,314)
(224,355)
(224,396)
(224,407)
(224,427)
(224,447)
(224,460)
(224,500)
(224,509)
(225,11)
(225,15)
(225,22)
(225,30)
(225,38)
(225,48)
(225,65)
(225,69)
(225,77)
(225,104)
(225,106)
(225,107)
(225,115)
(225,120)
(225,143)
(225,154)
(225,165)
(225,186)
(225,237)
(225,239)
(225,244)
(225,266)
(225,302)
(225,318)
(225,321)
(225,329)
(225,345)
(225,353)
(225,363)
(225,372)
(225,404)
(225,410)
(225,422)
(225,511)
(226,17)
(226,55)
(226,96)
(226,117)
(226,130)
(226,164)
(226,167)
(226,210)
(226,270)
(226,282)
(226,330)
(226,334)
(226,343)
(226,346)
(226,357)
(226,365)
(226,369)
(226,373)
(226,495)
(227,33)
(227,37)
(227,61)
(227,79)
(227,113)
(227,114)
(227,142)
(227,156)
(227,160)
(227,162)
(227,199)
(227,205)
(227,215)
(227,229)
(227,240)
(227,274)
(227,307)
(227,335)
(227,338)
(227,367)
(227,383)
(227,412)
(227,418)
(227,431)
(227,472)
(227,485)
(228,67)
(228,82)
(228,99)
(228,170)
(228,196)
(228,233)
(228,238)
(228,247)
(228,263)
(228,317)
(228,356)
(228,398)
(228,401)
(228,433)
(228,441)
(228,488)
(229,7)
(229,27)
(229,46)
(229,63)
(229,78)
(229,103)
(229,105)
(229,148)
(229,159)
(229,172)
(229,189)
(229,208)
(229,251)
(229,257)
(229,262)
(229,289)
(229,290)
(229,305)
(229,320)
(229,336)
(229,337)
(229,359)
(229,376)
(229,387)
(229,391)
(229,416)
(229,437)
(229,457)
(229,479)
(229,492)
(229,506)
(230,10)
(230,19)
(230,54)
(230,68)
(230,72)
(230,76)
(230,90)
(230,95)
(230,112)
(230,122)
(230,126)
(230,135)
(230,158)
(230,166)
(230,175)
(230,183)
(230,195)
(230,198)
(230,207)
(230,212)
(230,222)
(230,223)
(230,230)
(230,280)
(230,297)
(230,300)
(230,314)
(230,349)
(230,355)
(230,407)
(230,427)
(230,447)
(230,460)
(230,474)
(230,499)
(230,500)
(230,509)
(231,11)
(231,15)
(231,22)
(231,30)
(231,38)
(231,48)
(231,65)
(231,69)
(231,80)
(231,104)
(231,106)
(231,107)
(231,115)
(231,120)
(231,138)
(231,143)
(231,154)
(231,165)
(231,173)
(231,186)
(231,236)
(231,237)
(231,239)
(231,244)
(231,266)
(231,302)
(231,318)
(231,321)
(231,328)
(231,329)
(231,345)
(231,353)
(231,363)
(231,404)
(231,410)
(231,422)
(231,432)
(231,439)
(231,477)
(231,511)
(232,17)
(232,35)
(232,55)
(232,96)
(232,117)
(232,130)
(232,164)
(232,167)
(232,178)
(232,210)
(232,265)
(232,270)
(232,282)
(232,330)
(232,334)
(232,343)
(232,346)
(232,357)
(232,365)
(232,369)
(232,373)
(232,390)
(232,495)
(233,33)
(233,37)
(233,61)
(233,79)
(233,113)
(233,114)
(233,129)
(233,142)
(233,144)
(233,156)
(233,160)
(233,162)
(233,199)
(233,205)
(233,215)
(233,229)
(233,234)
(233,240)
(233,274)
(233,307)
(233,335)
(233,338)
(233,367)
(233,383)
(233,412)
(233,418)
(233,431)
(233,472)
(233,485)
(234,82)
(234,83)
(234,99)
(234,131)
(234,161)
(234,170)
(234,196)
(234,233)
(234,238)
(234,247)
(234,263)
(234,317)
(234,356)
(234,360)
(234,398)
(234,401)
(234,408)
(234,441)
(234,456)
(234,488)
(234,510)
(235,7)
(235,42)
(235,46)
(235,63)
(235,105)
(235,148)
(235,159)
(235,172)
(235,189)
(235,208)
(235,251)
(235,257)
(235,262)
(235,286)
(235,289)
(235,301)
(235,305)
(235,320)
(235,336)
(235,359)
(235,387)
(235,391)
(235,416)
(235,435)
(235,437)
(235,443)
(235,457)
(235,492)
(235,506)
(236,10)
(236,19)
(236,54)
(236,72)
(236,95)
(236,112)
(236,126)
(236,135)
(236,158)
(236,175)
(236,183)
(236,195)
(236,198)
(236,207)
(236,212)
(236,222)
(236,223)
(236,226)
(236,230)
(236,232)
(236,300)
(236,314)
(236,349)
(236,355)
(236,389)
(236,427)
(236,447)
(236,448)
(236,460)
(236,499)
(236,500)
(236,509)
(237,2)
(237,15)
(237,22)
(237,25)
(237,30)
(237,38)
(237,48)
(237,65)
(237,69)
(237,76)
(237,80)
(237,104)
(237,106)
(237,107)
(237,111)
(237,115)
(237,120)
(237,143)
(237,154)
(237,165)
(237,173)
(237,237)
(237,239)
(237,244)
(237,266)
(237,302)
(237,318)
(237,329)
(237,345)
(237,353)
(237,363)
(237,376)
(237,404)
(237,410)
(237,422)
(237,432)
(237,511)
(238,17)
(238,35)
(238,55)
(238,96)
(238,117)
(238,130)
(238,164)
(238,167)
(238,178)
(238,265)
(238,282)
(238,330)
(238,334)
(238,343)
(238,346)
(238,357)
(238,365)
(238,369)
(238,373)
(238,495)
(238,501)
(239,33)
(239,61)
(239,79)
(239,113)
(239,114)
(239,144)
(239,160)
(239,162)
(239,199)
(239,229)
(239,240)
(239,274)
(239,307)
(239,335)
(239,338)
(239,367)
(239,383)
(239,412)
(239,418)
(239,431)
(239,472)
(239,485)
};


==> mydefs.tex <==

\def\eqd{=_{\textup{\tiny{def}}}}

%
% important colors
%
\definecolor{steelblue1}{RGB}{99,184,255}
\definecolor{steelblue2}{RGB}{92,172,238}
\definecolor{steelblue3}{RGB}{79,148,205}
\definecolor{steelblue4}{RGB}{70,130,180}
\definecolor{steelblue5}{RGB}{54,100,139}



\renewcommand{\vec}[1]{\mathbf{#1}}


%\def\Netint{\Psi}
%\def\netint{\psi}


\def\Netact{\Phi}
\def\netact{\varphi}

\def\cellinact{f}
\def\celloutact{g}

\def\neterr{\epsilon}
\def\stateerr{\zeta}

\def\intersection{\vec{q}}
\def\sensororigin{\vec{o}}
\def\sensorrange{d}
\def\sensoraxis{\vec{a}}
\def\sensorvaluefunction{f}
\def\sensorvalue{v}
\def\sensorweight{\beta}
\def\sensorsmooth{\lambda}
\def\sensorvector{\boldsymbol{\upnu}}
\def\scv{\check{\vec{s}}}
\def\indeg{\operatorname{indeg}}
\def\outdeg{\operatorname{outdeg}}

\def\signsmooth{\alpha}



\def\scalepos{\gamma_{pos}}
\def\scalerot{\gamma_{rot}}
\def\scalesen{\gamma_{sen}}

%\def\netinput{\sigma}
\def\netinput{net} %  \upsilon}
\def\netoutput{x}

\def\trainset{S}
\def\testset{S'}
\def\validationset{S^{\ast}}

\newcommand{\tidx}[1]{#1}

\def\netinput{net}
\def\arminput{\upvarphi}
\def\netloss{\mathcal{L}}

